Fully Synthetic Data Improves Neural Machine Translation with Knowledge Distillation

This paper explores augmenting monolingual data for knowledge distillation in neural machine translation. Source language monolingual text can be incorporated as a forward translation. Interestingly, we find the best way to incorporate target language monolingual text is to translate it to the source language and round-trip translate it back to the target language, resulting in a fully synthetic corpus. We find that combining monolingual data from both source and target languages yields better performance than a corpus twice as large only in one language. Moreover, experiments reveal that the improvement depends upon the provenance of the test set. If the test set was originally in the source language (with the target side written by translators), then forward translating source monolingual data matters. If the test set was originally in the target language (with the source written by translators), then incorporating target monolingual data matters.

==> backup.tex <==


\begin{table*}[ht!]

\centering
% \usepackage{color}
% \usepackage{multirow}


\begin{tabular}{@{}l@{ ~}l@{ }|@{ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ }|ccc@{}}
\multicolumn{13}{l}{\textbf{BLEU by original language} }                                                                                                                                                                                                                                                                                       \\ 
\hline
& & \multicolumn{9}{c|}{Tr-En model}                                                                                                                                                                                                & \multicolumn{3}{c}{Et-En model}                                           \\
  &                             & \multicolumn{3}{@{ }c@{ }|}{WMT16}                                                & \multicolumn{3}{@{ }c|}{WMT17}                                                & \multicolumn{3}{c|}{WMT18}                                                & \multicolumn{3}{c}{WMT13}                                                 \\
  & Test original language=                              & src                      & tgt                     & all                   & src                      & tgt                      & all                   & src                      & tgt                      & all                   & src                      & tgt                      & all                   \\ 
\hline \hline
 \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small Training Data}}} & \textbf{Big Model  (781 MB)}                                                                                           & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
& ~~\para{} + \btp                             & 19.7                    & 28.2                    & 24.4                  & 18.7                    & 28.4                    & 23.9                  & 16.1                    & 32.2                    & 25.0                  & 28.2                    & 38.2                    & 33.6                  \\
& \textbf{Tiny Model (65 MB)}                     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}  \\
& ~~\para{} + \btp                              & 12.9                    & 17.0                    & 15.1                  & 12.3                    & 17.6                    & 15.0                  & 10.5                    & 19.2                    & 15.1                  & 25.1                    & 32.9                    & 29.5                  \\

%\textbf{Student:}                      & & & & & & & & & &  \\
& ~~\ft{\para{}+\btp}                              & {17.8}   & \textbf{24.2}  & 21.3                  & {16.6}   & \textbf{24.8}  & 20.7                  & {14.3}   & \textbf{27.8}  & 21.6                  & {26.4}   & \textbf{33.4}  & 30.3                  \\
& ~~\ft{\para{}+\mono{}}                              & \textbf{19.2}  & {22.3}   & 21.1                  & \textbf{18.3}  & {23.6}   & 21.1                  & \textbf{16.0}  & {26.6}   & 21.8                  & \textbf{28.6}  & {31.7}   & 30.6                  \\
& ~~\ft{\para{}+\mono{}+\btp}           & \textbf{19.7}  & \textbf{25.0}  & 22.6                  & \textbf{18.9}  & \textbf{25.8}  & 22.5                  & \textbf{16.2}  & \textbf{29.0}  & 23.1                  & \textbf{28.1}  & \textbf{34.5}  & 31.6                  \\
& ~~\ft{\para{}+\mono{}}\texttt{+}\btp & 19.2  & 24.3 & 22.2 & 18.6 & 24.9  & 22.0 & 15.7 & 27.6 & 22.4 & 27.8 & 33.1 &  30.9 \\
\hline
\end{tabular}

\rule{0pt}{2ex}    


\begin{tabular}{@{}l@{ ~}l@{ }|@{ }c@{ ~ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ ~ }c@{}} 
\hline
 &                                & \multicolumn{12}{c}{Es-En model}                                                                                                                                                                                                                                                                       \\
 &                             & \multicolumn{4}{c|}{WMT10}                                                                       & \multicolumn{4}{c|}{WMT11}                                                                       & \multicolumn{4}{c}{WMT12}                                                                        \\
& Test original language=& src                      & tgt                      & other                & all                   & src                      & tgt                      & other                & all                   & src                      & tgt                      & other                & all                   \\ 
\hline \hline
 \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small Training Data}}} &\textbf{Big Model (781 MB)}                                                                                             & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
&~~\para{} + \btp                                                                                                     & 43.9                    & 57.2                    & 27.7                 & 37.8                  & 41.1                    & 54.1                    & 25.7                 & 35.7                  & 53.0                    & 59.9                    & 25.5                 & 39.9                  \\
&\textbf{Tiny Model (65 MB)}                                                                                            & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
&~~\para{} + \btp                                                                                                     & 38.7                    & 53.1                    & 25.1                 & 34.4                  & 36.2                    & 49.4                    & 23.4                 & 32.3                  & 47.2                    & 54.3                    & 23.8                 & 36.5                  \\

&~~\ft{\para{}+\btp} & {41.8}  & \textbf{54.4} & 26.0                      & 35.7                     & {38.9}  & \color{worse}51.4 & \color{bad} 24.0 & 33.7                     & \color{best}51.2  & \color{better}{56.1} & \color{good}24.6                      & \color{ok}38.2                     \\
&~~\ft{\para{}+\mono{}}                                                                                                     & \textbf{42.9}  & {52.1}   & 26.6                 & 36.0                  & \textbf{41.2}  & {49.4}   & 24.5                 & 34.3                  & \textbf{52.8}  & {54.7}   & 25.0                 & 38.5                  \\
&~~\ft{\para{}+\mono{}+\btp}                                                                                  & \textbf{42.7}  & \textbf{54.4}  & 26.4                 & 36.1                  & \textbf{41.4}  & \textbf{50.4}  & 24.4                 & 34.4                  & \textbf{52.3}  & \textbf{56.0}  & 24.8                 & 38.6                  \\
& ~~\ft{\para{}+\mono{}}\texttt{+}\btp & 42.9 & 54.1 & 26.1 & 36.0 & 41.0 & 50.0 & 24.1 & 34.1 & 51.8 & 54.7 & 24.8 & 38.1 \\
\hline
\end{tabular}


\caption{Experiment results in terms of BLEU, divided based on the test-set's original language. The Big model is our teacher model. Models trained with forward-translated data (denoted with FT(...)) are our student models. For the training data, please refer to Table~\ref{tab:data-summary}.}
\label{main-res}
\end{table*}



==> table_main.tex <==

\begin{table*}[ht!]

\centering
% \usepackage{color}
% \usepackage{multirow}

\label{main-res}
\begin{tabular}{@{}l@{ }|@{ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ }|ccc@{}}
\multicolumn{13}{l}{\textbf{BLEU by original language} }                                                                                                                                                                                                                                                                                       \\ 
\hline
\multirow{3}{*}{Training data} & \multicolumn{9}{c|}{Tr-En model}                                                                                                                                                                                                & \multicolumn{3}{c}{Et-En model}                                           \\
                               & \multicolumn{3}{@{ }c@{ }|}{WMT16}                                                & \multicolumn{3}{@{ }c|}{WMT17}                                                & \multicolumn{3}{c|}{WMT18}                                                & \multicolumn{3}{c}{WMT13}                                                 \\
                               & tr                      & en                      & all                   & tr                      & en                      & all                   & tr                      & en                      & all                   & et                      & en                      & all                   \\ 
\hline \hline
% \textbf{Teacher:} ~~\para{} + \btp                     & & & & & & & & & &  \\
\textbf{Teacher:} \para{} + \btp                             & 19.7                    & 28.2                    & 24.4                  & 18.7                    & 28.4                    & 23.9                  & 16.1                    & 32.2                    & 25.0                  & 28.2                    & 38.2                    & 33.6                  \\
% \textbf{Tiny Model}                     & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}  \\
\textbf{Non-Student:} \para{} + \btp                              & 12.9                    & 17.0                    & 15.1                  & 12.3                    & 17.6                    & 15.0                  & 10.5                    & 19.2                    & 15.1                  & 25.1                    & 32.9                    & 29.5                  \\
\hline
\textbf{Student:}                      & & & & & & & & & &  \\
~~\ft{\para{}+\btp}                              & \textcolor{red}{17.8}   & \textcolor{blue}{24.2}  & 21.3                  & \textcolor{red}{16.6}   & \textcolor{blue}{24.8}  & 20.7                  & \textcolor{red}{14.3}   & \textcolor{blue}{27.8}  & 21.6                  & \textcolor{red}{26.4}   & \textcolor{blue}{33.4}  & 30.3                  \\
~~\ft{\para{}+\mono{}}                              & \textcolor{blue}{19.3}  & \textcolor{red}{22.6}   & 21.2                  & \textcolor{blue}{18.5}  & \textcolor{red}{24.0}   & 21.4                  & \textcolor{blue}{15.8}  & \textcolor{red}{27.1}   & 21.9                  & \textcolor{blue}{28.6}  & \textcolor{red}{31.7}   & 30.6                  \\
~~\ft{\para{}+\btp+\mono{}}           & \textcolor{blue}{19.8}  & \textcolor{blue}{25.7}  & 23.1                  & \textcolor{blue}{18.4}  & \textcolor{blue}{26.3}  & 22.6                  & \textcolor{blue}{15.9}  & \textcolor{blue}{29.6}  & 23.4                  & \textcolor{blue}{28.1}  & \textcolor{blue}{34.5}  & 31.6                  \\
\hline
\end{tabular}

\rule{0pt}{3ex}    


\begin{tabular}{@{}l@{ }|@{ }c@{ ~ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ ~ }c@{ }|c@{ ~ }c@{ ~ }c@{ ~ }c@{}} 
\hline
                                 & \multicolumn{12}{c}{Es-En model}                                                                                                                                                                                                                                                                       \\
                              & \multicolumn{4}{c|}{WMT10}                                                                       & \multicolumn{4}{c|}{WMT11}                                                                       & \multicolumn{4}{c}{WMT12}                                                                        \\
 \multirow{-3}{*}{Training data} & es                      & en                      & other                & all                   & es                      & en                      & other                & all                   & es                      & en                      & other                & all                   \\ 
\hline \hline
% \textbf{Big Model}                                                                                             & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
\textbf{Teacher:} \para{} + \btp                                                                                                     & 43.2                    & 57.2                    & 27.7                 & 37.3                  & 39.9                    & 54.2                    & 25.7                 & 35.2                  & 52.3                    & 59.8                    & 25.5                 & 39.7                  \\
% \textbf{Tiny Model}                                                                                            & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
\textbf{Non-Student:} \para{} + \btp                                                                                                     & 38.7                    & 53.1                    & 25.1                 & 34.4                  & 36.2                    & 49.4                    & 23.4                 & 32.3                  & 47.2                    & 54.3                    & 23.8                 & 36.5                  \\
\hline
\textbf{Student:}                      & & & & & & & & & &  \\
~~\ft{\para{}+\btp} & \textcolor{red}{41.8}  & \textcolor{blue}{54.4} & 26.0                      & 35.7                     & \textcolor{red}{38.9}  & \textcolor{blue}{51.4} & 24.0 & 33.7                     & \textcolor{red}{51.2}  & \textcolor{blue}{56.1} & 24.6                      & 38.2                     \\
~~\ft{\para{}+\mono{}}                                                                                                     & \textcolor{blue}{42.9}  & \textcolor{red}{52.1}   & 26.6                 & 36.0                  & \textcolor{blue}{41.2}  & \textcolor{red}{49.4}   & 24.5                 & 34.3                  & \textcolor{blue}{52.8}  & \textcolor{red}{54.7}   & 25.0                 & 38.5                  \\
~~\ft{\para{}+\btp+\mono{}}                                                                                  & \textcolor{blue}{42.7}  & \textcolor{blue}{54.4}  & 26.4                 & 36.1                  & \textcolor{blue}{41.4}  & \textcolor{blue}{50.4}  & 24.4                 & 34.4                  & \textcolor{blue}{52.3}  & \textcolor{blue}{56.0}  & 24.8                 & 38.6                  \\
\hline
\end{tabular}


\caption{Experiment results in terms of BLEU, divided based on the test-set's original language. The teachers are trained with \texttt{Big} model. Non-students are trained with the same \texttt{Tiny} model architecture as the student, except that they are trained from scratch (no knowledge distillation). For the training data, please refer to Table~\ref{tab:data-summary}.}
\label{main-res}
\end{table*}



==> table_tmp.tex <==

\begin{table*}
\small
\centering
\begin{tabular}{ll@{ }|c@{~~~ }c@{~~~ }c|c@{~~~ }c@{~~~ }c|c@{~~~ }c@{~~~ }c|c@{~~~ }c@{~~~ }c}
\multicolumn{14}{l}{\textbf{BLEU by original language}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                                                                                             & {\cellcolor[rgb]{0.937,0.937,0.937}}                                & \multicolumn{9}{c|}{Tr-En model}                                                                                                                                                                                                           & \multicolumn{3}{c}{Et-En model}                                              \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                                                                                                             & {\cellcolor[rgb]{0.937,0.937,0.937}}                                & \multicolumn{3}{c|}{WMT16}                                           & \multicolumn{3}{c|}{WMT17}                                           & \multicolumn{3}{c|}{WMT18}                                           & \multicolumn{3}{c}{WMT13}                                            \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-3}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.937,0.937,0.937}}l@{}} Model\\size \end{tabular}} & \multirow{-3}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}Training data} & tr & en & all &  tr & en & all &  tr & en & all &  et & en & all  \\ 

Big                                                                                                                                                                                & \para{} + \btp                                                          & 19.7                    & 28.2                    & 24.4                     & 18.7                    & 28.4                    & 23.9                     & 16.1                    & 32.2                    & 25.0                     & 28.2                    & 38.2                    & 33.6                     \\ \hline
Tiny                                                                                                                                                                               & \para{} + \btp                                                          & 12.9                    & 17.0                    & 15.1                     & 12.3                    & 17.6                    & 15.0                     & 10.5    & 19.2   & 15.1    & 25.1  & 32.9    & 29.5     \\
                                                                                                                                                                                   & \ft{\para{} + \btp}                                              & \textcolor{red}{17.8}   & \textcolor{blue}{24.2}  & 21.3                     & \textcolor{red}{16.6}   & \textcolor{blue}{24.8}  & 20.7                     & \textcolor{red}{14.3}   & \textcolor{blue}{27.8}  & 21.6                     & \textcolor{red}{26.4}   & \textcolor{blue}{33.4}  & 30.3                     \\
                                                                                                                                                                                   & \ft{\para{} + \mono{}}                                            & \textcolor{blue}{19.3}  & \textcolor{red}{22.6}   & 21.2                     & \textcolor{blue}{18.5}  & \textcolor{red}{24.0}   & 21.4                     & \textcolor{blue}{15.8}  & \textcolor{red}{27.1}   & 21.9                     & \textcolor{blue}{28.6}  & \textcolor{red}{31.7}   & 30.6                     \\
                                                                                                                                                                                   & \ft{\para{} + \btp~+ \mono{}}                                      & \textcolor{blue}{19.8}  & \textcolor{blue}{25.7}  & 23.1                     & \textcolor{blue}{18.4}  & \textcolor{blue}{26.3}  & 22.6                     & \textcolor{blue}{15.9}  & \textcolor{blue}{29.6}  & 23.4                     & \textcolor{blue}{28.1}  & \textcolor{blue}{34.5}  & 31.6                    
                                                                                                                                                                                   \\ \hline
\end{tabular}
\rule{0pt}{3ex}    



\begin{tabular}{ll@{ }|c@{~~~ }c@{~~~ }c@{~~~ }c|c@{~~~ }c@{~~~ }c@{~~~ }c|c@{~~~ }c@{~~~ }c@{~~~ }c}
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                        & {\cellcolor[rgb]{0.937,0.937,0.937}}                           & \multicolumn{12}{c}{ES-EN model}                                                                                                                                                                                                                                                                                                \\
\rowcolor[rgb]{0.937,0.937,0.937} {\cellcolor[rgb]{0.937,0.937,0.937}}                        & {\cellcolor[rgb]{0.937,0.937,0.937}}                           & \multicolumn{4}{c|}{WMT10}                                                                             & \multicolumn{4}{c|}{WMT11}                                                                                    & \multicolumn{4}{c}{WMT12}                                                                              \\
\rowcolor[rgb]{0.937,0.937,0.937} \multirow{-3}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.937,0.937,0.937}}l@{}} Model\\size \end{tabular}} & \multirow{-3}{*}{{\cellcolor[rgb]{0.937,0.937,0.937}}Training data} & es & en & other & all & es & en & other & all & es & en & other & all \\
Big                                                                                           & \para{} + \btp                                                     & 43.2                   & 57.2                   & 27.7                      & 37.3                     & 39.3                   & 54.2                   & 25.7                             & 35.2                     & 52.3                   & 59.8                   & 25.5                      & 39.7                     \\ \hline
Tiny                                                                                          &  \para{} + \btp                                                     & 38.7                   & 53.1                   & 25.1                      & 34.4                     & 36.2                   & 49.4                   & 23.4                             & 32.3                     & 47.2                   & 54.3                   & 23.8                      & 36.5                     \\
                                                                                              & \ft{\para{} + \btp}                                         & \textcolor{red}{41.8}  & \textcolor{blue}{54.4} & 26.0                      & 35.7                     & \textcolor{red}{38.9}  & \textcolor{blue}{51.4} & 24.0 & 33.7                     & \textcolor{red}{51.2}  & \textcolor{blue}{56.1} & 24.6                      & 38.2                     \\
                                                                                              & \ft{\para{} + \mono{}}                                       & \textcolor{blue}{42.9} & \textcolor{red}{52.1}  & 26.6                      & 36.0                     & \textcolor{blue}{41.2} & \textcolor{red}{49.4}  & 24.5 & 34.3                     & \textcolor{blue}{52.8} & \textcolor{red}{54.7}  & 25.0                      & 38.5                     \\
                                                                                          & \ft{\para{} + \btp ~+ \mono{}}                                  & \textcolor{blue}{42.7} & \textcolor{blue}{54.4} & 26.4                      & 36.1                     & \textcolor{blue}{41.4} & \textcolor{blue}{50.4} & 24.4 & 34.4                     & \textcolor{blue}{52.3} & \textcolor{blue}{56.0} & 24.8                      & 38.6     
                                                                                          \\ \hline
\end{tabular}


\caption{Experiment results in terms of BLEU, divided based on the test-set's original language. The Big model is our teacher model. Models trained with forward-translated data (denoted with FT(...)) are our student models. For the training data, please refer to Table~\ref{tab:data-summary}.}
\label{main-res}
\end{table*}


